Learning Robust Representations by Projecting Superficial Statistics Out

Despite impressive performance as evaluated on i.i.d. holdout data, deep neural networks depend heavily on superficial statistics of the training data and are liable to break under distribution shift. For example, subtle changes to the background or texture of an image can break a seemingly powerful classifier. Building on previous work on domain generalization, we hope to produce a classifier that will generalize to previously unseen domains, even when domain identifiers are not available during training. This setting is challenging because the model may extract many distribution-specific (superficial) signals together with distribution-agnostic (semantic) signals. To overcome this challenge, we incorporate the gray-level co-occurrence matrix (GLCM) to extract patterns that our prior knowledge suggests are superficial: they are sensitive to the texture but unable to capture the gestalt of an image. Then we introduce two techniques for improving our networks' out-of-sample performance. The first method is built on the reverse gradient method that pushes our model to learn representations from which the GLCM representation is not predictable. The second method is built on the independence introduced by projecting the model's representation onto the subspace orthogonal to GLCM representation's. We test our method on the battery of standard domain generalization data sets and, interestingly, achieve comparable or better performance as compared to other domain generalization methods that explicitly require samples from the target distribution for training.

==> discussion.tex <==
\subsection{Parameter Tuning Heuristics}
There are several parameter tuning heuristics that can be used to improve the performance of HEX. 

For example, at the beginning, we do not train with HEX until the model gets stable. 

Also, since the NGLCM will inevitably learn some semantic information, we can choose to not update the weights of after certain epochs of NGLCM. 

In our experiments, to show the performance of the idea of HEX, we did not employ any of these heuristics except the one introduced in the PACS experiment. 

\subsection{Hyperparameter Choices of NGLCM}
There are two hyperparameters of NGLCM: the number of gray levels (we chose 16 in the experiment to reduce number of parameters), and the direction (we chose $\dag{0}$ as the most natural choices). For fair comparison, we did not tune these hyperparameters through these experiments. 

\subsection{When the matrix $F_G^TF_G$ is not invertible}
When the matrix $F_G^TF_G$ in Equation~\ref{eq:hex} is not invertible, we use heteroscadestic regression instead. We name our method ``HEX'' as a short of ``heteroscadestic''. 

\subsection{Applying HEX on i.i.d data}
We also try the idea of HEX on standard MNIST data, the performance slightly drops. We believe the reason is that NGLCM will inevitably learn some semantic information and HEX projects the information learned by NGLCM out and lowers the overall performance as a result. 
